Configuration Validation with Large Language Models

Misconfigurations are major causes of software failures. Existing practices rely on developer-written rules or test cases to validate configurations, which are expensive. Machine learning (ML) for configuration validation is considered a promising direction, but has been facing challenges such as the need of large-scale field data and system-specific models. Recent advances in Large Language Models (LLMs) show promise in addressing some of the long-lasting limitations of ML-based configuration validation. We present a first analysis on the feasibility and effectiveness of using LLMs for configuration validation. We empirically evaluate LLMs as configuration validators by developing a generic LLM-based configuration validation framework, named Ciri. Ciri employs effective prompt engineering with few-shot learning based on both valid configuration and misconfiguration data. Ciri checks outputs from LLMs when producing results, addressing hallucination and nondeterminism of LLMs. We evaluate Ciri's validation effectiveness on eight popular LLMs using configuration data of ten widely deployed open-source systems. Our analysis (1) confirms the potential of using LLMs for configuration validation, (2) explores design space of LLMbased validators like Ciri, and (3) reveals open challenges such as ineffectiveness in detecting certain types of misconfigurations and biases towards popular configuration parameters.

==> figs/code.tex <==
\begin{minted}[fontsize=\footnotesize, linenos=false, frame=none, xleftmargin=0.2em, xrightmargin=5em]{python}
    try:
        with open("/path/to/file", "r") as f:
            data = json.loads(f.read())
            print("Valid configuration")
    except:
        print("Invalid configuration")
    \end{minted}
    

==> sections/finding-v0.tex <==
\section{Evaluation and Findings}
\label{sec:finding}

\subsection{Overall Effectiveness}

% \jie{The findings still need to be better summarized and organized. It is also better if you can present findings with results. See an example on \url{https://arxiv.org/abs/2205.12628}.}

% \subsection{Observation1: The different design of the \ourframework has
% huge impact on the effectiveness}

% \jie{The titles of Observation 1 and Observation 2 are too general and obvious. They do not contain any meaningful information.}

% \finding{The effectiveness of \llms is influenced by both number of 
% valid configuration shots and misconfiguration shots.}
% \finding{The performance of \ourframework is influenced by a balance between the \faultyconfig and \validconfig examples. Incorporating \validconfig examples effectively reduces the FP cases, whereas an increased emphasis on \faultyconfig diminishes the FN cases.}

% \finding{\faultyconfig shots are more foundational to \ourframework's effectiveness in discerning \misconfigs than \validconfig shots; but a balanced integration of both \faultyconfig and \validconfig shots is crucial for optimal performance}

% ====================
\finding{\ourframework demonstrates promises in using large language models (\llms) as configuration validators.
    It effectively achieves file-level and parameter-level F1-scores of up to 0.75 and 0.56, respectively, in our configuration dataset.}
% \xinyu{Table 5 and Table 6 have inconsistent title. One is '\fw', the other one is 'LLMs'}
\ourframework exhibits remarkable capability in \config validation, as shown in Table~\ref{tab:overview}. 
It not only identifies the \misconfig files,
    but also pinpoints the erroneous parameters 
    and ascertain the underlying causes of the \misconfigs. 
However, the choice of the \llms is crucial. 
The GPT base models~\cite{openaimodels}, 
    supported by the legacy GPT-3 model and 
    not optimized for instruction-following, 
    has limited capability in in \misconfig detection.
For example, Davinci-002 only achieves a parameter-level F1-score of 0.09, 
    significantly lower than the others.
Another evaluated base model, Babbage-002, 
    fails to detect any \misconfig, 
    consistently deeming incoming \config files as valid.

\input{tables/finding1.tex}

\phantomsection\finding{Directly applying \llms as configuration validators 
    has both non-trivial false negatives and false positives. 
    For instance, both GPT base models (Davinci-002 and Babbage-002) do not detect any \misconfig,
    and \gptdavinci's F1-scores plunge to as low as 0.08.}
\label{finding:2}
\input{tables/finding2.tex}
Configuration shots play an important role in influencing the performance of LLMs. 
In scenarios where no \config shots are supplied, 
    \gptturbo manages a parameter-level F1-score of 0.24,  
    while \gptdavinci performs worse with a mere 0.08, as illustrated in Table~\ref{tab:weekness}.
The parameter-level precision of these two models is 0.16 and 0.08, respectively. 
This indicates a significant volume of false positives when detecting \misconfig. 
As for false negatives, \gptdavinci has a recall of 0.09, 
    suggesting a non-trivial presence of undetected \misconfigs.
Notably, the \gptfour model, though being slower and more expensive to use, 
    distinguishes itself in \config validation tasks. 
Despite being over 20 times more expensive than \gptturbo~\cite{openaipricing},
    even in the absence of \config shots, 
    it delivers a parameter-level F1-score of 0.47, 
    showing its great generalization capabilities.
This suggests that, when budget allows, 
    investing in a more advanced model such as \gptfour 
    can yield superior results, 
    emphasizing the critical role of model selection again.

% \yf{Show how we calculate the avg F1. - resolved in metric section}
% \yf{Shall we add another finding for GPT-4 here?}

\subsection{All About Shots}
\label{subsection:shot}
\ourframework's effectiveness is greatly influenced by combination of 
    the ValidConfig and Misconfig shots.
To explore the optimal strategy for shot file selection, 
    we conduct a series of experiments with different shot file combinations.
For the sake of manageability and cost-effectiveness,
    we randomly select three projects: \hbase, \hcommon, and \alluxio, 
    by using two models: \gptturbo and \gptdavinci,
    as testing all six projects and five models would be prohibitively expensive.

\phantomsection\finding{Few-shot learning with labeled configuration data, 
    including both ValidConfig 
    and Misconfig, can significantly improve configuration validation effectiveness.
    For example, when provided with four shots (one ValidConfig shot and three Misconfig shots), 
    \gptdavinci achieves its optimal parameter-level F1-score.}
    \label{finding:3}

\phantomsection\finding{Labeled Misconfig, 
    despite being significantly lacking in practice, 
    are crucial to validation effectiveness of \ourframework.
    Relying solely on ValidConfig, 
    \gptturbo does not achieve parameter-level F1-scores higher than 0.25.
    However, when Misconfig shots are introduced, 
        \gptturbo's F1-scores consistently exceed above 0.35.}
\label{finding:4}
    
% Guidance \faultyconfig in the form of ``shots'' are foundational to \ourframework's effectiveness.}
As shown in Figure~\ref{fig:heatmapcodex}-\ref{fig:heatmapturbo}, 
    Misconfig shots allow \ourframework to more effectively identify 
    patterns and attributes commonly associated with \misconfigs, 
    surpassing the capabilities offered by ValidConfig. 
In the absence of labeled Misconfig, 
    the ability of \ourframework becomes limited. 
With \gptdavinci, \ourframework only gets an F1-score of approximately 0.2 
    (as denoted by the first column of the heat map), 
    when only using ValidConfig shots in the prompt. 

Only relying on labeled Misconfig can also inadvertently bias the model,
    since the input text distribution significantly impacts 
    the performance of \llms~\cite{min:arxiv:22}.
In our evaluation, there is not a direct correlation 
    between the number of ValidConfig shots and the reduction in FP or FN cases
    e.g., the FP reduction rate is directly proportional 
    to the number of ValidConfig shots. 
However, introducing the ValidConfig shot does reduce FP cases for \gptdavinci
    and FN cases for \gptturbo.
This indicates that, by incorporating both Misconfig and ValidConfig, 
    \ourframework gains a more balanced perspective. 
    % enabling it to discern between \misconfigs and valid \configs 
    % that might superficially resemble an erroneous pattern. 

\input{figs/heatmap.tex}

\phantomsection\finding{It is challenging, but also crucially important, 
        to achieve a balanced integration of ValidConfig  
    and Misconfig in few-shot learning. 
    Otherwise, the \llms will become biased.
    Both \gptturbo and \gptdavinci achieve their highest F1 scores 
    when provided with one ValidConfig and three Misconfig shots.}
\label{finding:5}

Due to the prohibitive cost and strict rate limit associated with \gptfour, 
    the exhaustive experiment of different shot combinations for \gptfour was not conducted.
Instead, we test it with only one setting, 
    i.e., one ValidConfig and three Misconfig shots,
    which is the same as the best setting for \gptturbo and \gptdavinci,
    since we believe that this setting is likely to be effective for \gptfour. 
If not specified, the following experiments are also done with this setting.
Note that, though \gptfour has already performed quite well, 
    it may achieve better results with alternative shot settings.

The Finding 3, 4 and 5 emphasize the importance of a holistic prompt examples 
    including both ValidConfig and Misconfig, 
    since over-relying on just one type of shot might compromise \ourframework.    

% \finding{The effectiveness of \ourframework is greatly influenced by the shot file selection strategy. Both Diff-Category and Similarity selection individually contribute to effectiveness. However, the hybrid 'Diff-Category + Similarity' method stands out as the most effective.}

% \finding{\tianyin{I don't understand this finding} Both Diff-Category and Similarity shot file selection strategies individually contribute to \ourframework's effectiveness, and the hybrid of these two methods stands out as the most effective.}

% \jie{Just providing an example here: You need to summarize/rephrase the findings to a more high-level/abstract finding. E.g., 

% high-level finding: the selection of in-context examples is important.

% Sub-findings: 1) Diversity; 2) Similarity/Relevance; 3) ...}

% \jie{Related works on in-context example selection: \url{https://aclanthology.org/2022.deelio-1.10/}, \url{https://openreview.net/forum?id=qY1hlv7gwg}}

% \finding{When the shot is selected from the same project, \llms demonstrate considerably better effectiveness than others scenarios.}

\phantomsection\finding{Leveraging configuration data from different projects as shots, 
    especially when the target project's data is unavailable, 
    showcases the transferability of \ourframework.
    For instance, when using \configs from other projects as shots for \hcommon's validation, 
    \ourframework maintains acceptable effectiveness, 
    achieving a parameter-level F1-score up to 0.44.}
    \label{finding:6}
% \yf{I found this finding is awkward. It is lower than the zero-shot..}
In scenarios where accessing configuration data 
    from a specific project might be challening,
    \ourframework's transferability becomes crucial.
To evaluate this transferability,
    the experiment is designed to use the shot files 
    from projects that are distinct from the target.

% Both \hcommon and \hbase, products of Apache and developed around the same time, 
%     share a common \config API. 
% This stands in contrast to \alluxio, making the latter a different entity. 
% Besides, both \hcommon and \hbase adopt the XML format for \config, 
%     while the \alluxio is using the key-value pair format.

The results in Table~\ref{tab:cross-system} emphasizes 
    a critical aspect of \ourframework: 
    the ability to apply knowledge across different systems.  
While there's a decline in effectiveness 
    when compared to using \hcommon's native \configs as shots, 
    \ourframework still manages to achieve acceptable F1-scores. 
For models like \gptturbo and \gptdavinci, 
    their efficacy surpasses that of zero-shot learning 
    (as shown in Table~\ref{tab:weekness}). 
In contrast, for \gptfour, regardless of the project, 
    its performance consistently falls short of 
    its zero-shot learning (F1-score 0.53).
This observation hints that, for advanced models like \gptfour,
    it is better to not use shots than 
    using shots from other projects,
    as the latter could introduce more biases.
% In the rapidly evolving cloud landscape, it's essential for tools like \ourframework 
%     to not just excel within a singular project 
%     but also demonstrate adaptability when introduced to others.

% \xinyu{The reason to do provide the shot from hadoop and hbase to alluxio in our experiment:
% 1) both hadoop and hbase is from apache and share the same config api, while the alluxio are quite different.
% 2) both hadoop and hbase is using the xml format for config file, while the alluxio is using the properties format that is in pure key-value pair.
% 3) the first version of hadoop is released in 2007 and hbase is in 2008 while the alluxio is in 2016.
% 4) the average G-hits of Hadoop's parameters is 1767, hbase is 1752, while the alluxio is 86.

% We want to show that even though the target project is quite different from the shot project (config file format is diff, api is diff, belong to diff org, quite new), \ourframework can still achieve a high level of effectiveness.}

\input{tables/cross-system.tex}
% \finding{Leveraging the probabilities of tokens to establish the threshold has proven advantageous.

% \finding{Providing detailed descriptions of configuration parameters seemed to impede rather than improve the effectiveness of LLMs.}

% \jie{Like what we discussed before, this may due to the variance or prompt design. A good finding needs to be generalized and not specific to a model and a prompt.}

% \sam{Because some people might be skeptical on whether some design choice findings can be generalized, spend some text sharing your experience on how to deal with these design complexity, and providing more implications are perhaps more useful to other system practitioners.}
% \sam{I suggest you first rewrite the evaluation subsections (which I believe are your ``observation'') into three RQs, for organizing your study results}

\subsection{When Do Things Go South}
% \yf{Need to emphasize that we use the 1-3 setting for the experiment somewhere.}
\finding{As the number of parameters increases in the \config file under test, the effectiveness of \ourframework decreases.}
As shown in Figure~\ref{fig:numparam}, this decline in \ourframework's performance 
    can be attributed to a potential information overload for \llms. 
As the complexity of the \config file grows, 
    the potential combinations and dependencies 
    between \config parameters also grow exponentially. 
    the model may struggle to process and understand the complex relationships 
    between the increasing number of parameters.
For instance, when the number of parameters jumps from 8 to 16, 
the performance of \ourframework begins to deteriorate severely.
This trend mirrors the challenges faced in other domains 
    where models are presented with an abundance of information, 
    often leading to decreased performance 
    as essential data become obscured amidst the surrounding noise.
\yf{@Jie, are there any references to support my point? If there is no reference, I will revise the last sentence.}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/numParam.pdf}
    \caption{Effectiveness of GPT-3.5-turbo across different number of parameters in the \config file under test.}
    \label{fig:numparam}
\end{figure}


% \finding{Our study of X types of misconfigurations revealed that without any supplementary information, LLMs can effectively identify {Y/X} of them. }

\finding{\ourframework excels in pinpointing \misconfigs in most sub-categories (12 out of 15), 
    but does not show the same proficiency for dependable and version categories.}

Table~\ref{tab:result_category} shows the effectiveness of 
    \ourframework in identifying various types of \misconfigs.
\sam{move this to here as xinyu said it's only used here: For the average F1 score, we resort to the macro F1, which is a more balanced metric.}
A closer inspection reveals that for the sub-categories: 
    Control, Value Relationship, and Parameter Change, 
    \ourframework's F1-scores do not surpass the 0.30.
This performance is significantly lower than other categories.
Notably, only \gptfour achieves a slightly better F1-score of 0.46 
    for the Value Relationship, 
    but this too falls short of its performance in others.
% To give equal weight to each \config in the same sub-category regardless of its project,
Note that, to focus on the same sub-category instead of the project, 
    we calculate the micro F1-score for the average.

The difference in performance can be attributed to 
    the inherent nature of the \misconfigs themselves. 
Sub-categories like Syntax and Range are more universal 
    and are areas where \llms have learned extensive knowledge from diverse sources. 
% These types of misconfigurations are akin to general computer science knowledge, 
%     which even a person with basic training can detect.
On the other hand, Dependency and Version categories are more project-specific. 
They are closely linked to the specific details of individual projects, 
    making them harder for models without extensive training on that project's data.
While general computer science knowledge might suffice to spot Syntax or Range errors,
    detecting \misconfigs related to dependencies or versioning would likely 
    require the expertise of the model deeply familiar with the project.
This distinction underscores the challenges faced by \ourframework 
    and highlights the importance of context-specific knowledge in \config validation.
\yf{@Xinyu, case study here.}
% \yf{Possible reasons why they are poor: 1. Complexity and Ambiguity; 2. Lack of training data.
% Consider comparing these with human's validation ability for these categories;
% and also case study here.}

% *use a vinn figure here for three models to see the difference on different types or parameters.
% \yf{@Xinyu, calculate avg for these three models.}
% \yf{Here the F1 is micro F1 since the different categories have different number of parameters.}
\input{tables/result_over_category.tex}

% \finding{\llms sometimes pinpoint parameters even if they are set to their default values.}
\finding{Despite LLMs being aware of default parameter values, they occasionally flag these default settings as misconfigurations during detection tasks.}
\yf{@Xinyu, calculate percentage for the default value that LLMs know.}

We query LLMs to determine their awareness of default parameter values. 
For each LLM, we calculate the percentage of default values they correctly answer. 
\gptfour, \gptturbo, and \gptdavinci are aware of the \yf{XX, XX, XX} default values respectively.
The goal is to ascertain if \fw could correctly identify 
    these default settings without flagging them as misconfigurations. 
Surprisingly, even with the high percentage of their knowledge 
    about the default value of some parameters, 
    LLMs still occasionally misinterpreted these default values.
As illustrated in Table~\ref{tab:default_v}, 
    there isn't a consistent pattern between 
    the mis-detection of default values and non-default values; 
    both can be erroneously flagged by LLMs.

\yf{I think the avg is also a macro avg for percentage? @Xinyu}
\yf{Case study?}
 \input{tables/default_v.tex}
% \input{tables/pinpoint_default.tex}

\finding{X\% reasons provided by the \llms are not comprehensible or not relevant to the misconfigurations. }
\yf{@Sam @Xinyu. Waiting for the result.
show one or two examples here, and try to explain why they reason badly for the case.}
% \subsection{Observation3: \llms have bias towards parameters based on their popolarity.}

% \finding{Within valid \conffiles, \llms are more likely pinpoint those parameters with higer G-hints.}

% \finding{When evaluated using the \validconfig dataset, \llms are more inclined to target parameters with higher G-hints.}

\finding{Upon evaluation with the ValidConfig dataset, 
    \ourframework leans more towards parameters that have higher G-hits, 
    indicating a direct correlation between a parameter's popularity in Google searches 
    and the likelihood of the LLM addressing it.}

% Definition of G-hits:
\textbf{G-hits}: A metric quantifying the prevalence of a specific keyword based on its appearances in Google search results. Specifically, G-hits index denotes the number of exact-match search results returned by Google for a keyword. 

As demonstrated in Figure~\ref{fig:Ghits Correct}, parameters within the \config 
    under examination are ranked based on their corresponding G-hits index. 
For the ValidConfig dataset, we counted the frequency with which \ourframework 
    identifies each ranked parameter. 
Specifically, we recorded how often \ourframework targets the parameter ranked first by G-hits, 
    the parameter ranked second, and so forth. 
If \ourframework marks multiple parameters as \misconfigs when testing a single \config file, 
    frequency will be distributed evenly across all of them.
Intriguingly, the distribution reveals a clear skewness towards parameters 
    with higher G-hits rankings. 
This trend can be attributed to the nature of the training data for \llms. 
Training data is often sourced from publicly accessible domains easily accessible 
    by search engine like Google\xinyu{Need to add reference}\yf{@Jie}, 
    which significantly influences \llms behavior. 
Popular topics or parameters are more likely embedded deeply into 
    the model's knowledge due to their prevalence in the training data.
% \xinyu{We may also need to mention that when there are multiple parameters in the result, we will distribute the weights accordingly.}


\input{figs/ghit.tex}

Ranked with G-hints, $8^{th}$ parameter is pinpointed 23 times. $1^{st}$ parameter is pinpointed 73 times.


% \finding{Within invalid \conffiles, \llms demonstrate enhanced accuracy in detecting invalid value of parameters with higher G-hints.}

\finding{When evaluated using the labeled \misconfig dataset, 
    \ourframework exhibits greater precision in identifying incorrect values 
    for parameters that have higher G-hints.}
In the evaluation of the labeled Misconfig dataset, 
    we observe a trend: 
parameters with higher G-hints, indicating their prevalence in search results, 
    are more accurately identified by \ourframework when they have incorrect values. 
Specifically, the median G-hits value 
    for correctly detected misconfigurations 
    is notably higher than that for misconfigurations 
    that \ourframework fails to identify. 


% \yf{Box plot please. @Xinyu}
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figs/box_figure.pdf}
    \caption{Distribution of G-hits for misconfigured parameters. 
    Left box represents G-hits distribution of parameters correctly detected, 
    while right box indicates the distribution of parameters that are failed to detect. 
    \yf{Polish this fig: the x-axis font is too small and non-bold.
        Use diff color for the two median. Fill the box with diff color and patterns.}}
    \label{fig:Ghits Wrong}
\end{figure}

% \finding{Bias on the parameter's non-default value: X\% false positives generated by LLMs can be attributed to X, i.e., LLMs tend to pinpoint parameters whose values deviate from their default values more frequently.}

% \finding{Bias on new projects beyond the training dataset: LLMs exhibited noticeably reduced effectiveness on new projects that they are not trained on. } 

% \jie{Haven't seen the results yet. Need to provide some quantitative analysis on the data/corpus to support the findings.}





==> sections/finding-v1.tex <==
\section{Evaluation and Findings}
\label{sec:finding}
In this section, we first present results on evaluating the effectiveness of \llms as configuration validators under \ourframework (\S\ref{sec:eval:overall}). 
We then analyze how \ourframework' configuration validation effectiveness change in relation to the provided shots under few-shot learning scenarios (\S\ref{sec:eval:shot}). 
In the following \S\ref{sec:eval:bias}, we present our understanding on when \ourframework can produce wrongful validation outcomes, and why these wrongful outcomes are produced due to potential bias originated from \llms' training; we also present a qualitative analysis on the reasonings return from \llms during configuration validation.

\subsection{Overall Effectiveness}
\label{sec:eval:overall}
% \jie{The findings still need to be better summarized and organized. It is also better if you can present findings with results. See an example on \url{https://arxiv.org/abs/2205.12628}.}

% \finding{\misconf shots are more foundational to \ourframework's effectiveness in discerning \misconfigs than \validconfig shots; but a balanced integration of both \misconf and \validconfig shots is crucial for optimal performance}

% ========================================
\finding{\ourframework demonstrates the effectiveness of using state-of-the-art \llms as configuration validators.
    It achieves \filelevel and \paramlevel F1-scores of up to 0.75 and 0.56, respectively. \label{finding:overall}}
\noindent
\ourframework exhibits remarkable capability in \config validation, 
    as shown in Table~\ref{tab:overview}.
% All \llms achieve 0.62-0.75 in average \fonescore across \numprojects projects at \filelevel.
Beyond merely identifying \misconfig files, 
    with an average \fonescore ranging from 0.62 to 0.75, 
    it also pinpoints erroneous parameters 
    and discerns the causes of the \misconfigs.
% It not only identifies the \misconfig files,
%     achieving 0.62-0.75 in average \fonescore,
%     but also pinpoints the erroneous parameters 
%     and ascertain the underlying causes of the \misconfigs. 
% For all \llms, the \recall is higher than \precision at both file and parameter levels, which indicates that \llms are inclined to report false alarms compared to missing actual misconfigurations. 
% Meanwhile, among the top-three \llms, the \paramlevel \fonescore{}s are about 25\% lower than their \filelevel counterparts. \sam{this is because...}
 
However, when using older models, we observe they lack 
    ability of effective configuration validation.
Specifically, for \davinci, its \fonescore has a sharp drop from \filelevel (0.63) to \paramlevel (0.09), 
    indicating that it is not able to localize the actual misconfigured parameter accurately. 
One reason is that \davinci lacks optimization for instruction-following, 
    leading it to occasionally produce inappropriate results. 
Furthermore, our evaluation of \babbage, a smaller model, reveals its inability to configuration validation. 
    It consistently regards every configuration file as correct, so it is omitted from Table~\ref{tab:overview}.

\para{Implication.} 
Our result suggests that the state-of-the-art \llms (e.g., \gptfour, \gptturbo) can be applied to configuration validation under properly designed framework (e.g., few-shot learning, voting from \ourframework), and achieve promising valdiation accuracy. However, older \llms (e.g., \davinci, \babbage) are often incapable for configuration validation due to insufficient training data and/or outdated training mechaisms. 
\llms tend to report more false alarms than missing misconfiguration, they are potentially useful in validation settings where the to-be-validated configurations can cause severe consequences (data loss, security breach) if misconfigured.
%\ourframework exhibits remarkable capability in \config validation, as shown in Table~\ref{tab:overview}. 
%It not only identifies the \misconfig files,
%    but also pinpoints the erroneous parameters 
%    and ascertain the underlying causes of the \misconfigs. 
%However, the choice of the \llms is crucial. 
%The GPT base models~\cite{openaimodels}, 
%    supported by the legacy GPT-3 model and 
%    not optimized for instruction-following, 
%    has limited capability in in \misconfig detection.
%For example, Davinci-002 only achieves a parameter-level F1-score of 0.09, 
%    significantly lower than the others.
%Another evaluated base model, \babbage, 
%    fails to detect any \misconfig, 
%    consistently deeming incoming \config files as valid.

\input{tables/finding1.tex}


% \phantomsection\finding{Directly applying \llms as configuration validators 
%     has both non-trivial false negatives and false positives. 
%     For instance, both GPT base models (Davinci-002 and Babbage-002) do not detect any \misconfig,
%     and \gptdavinci's F1-scores plunge to as low as 0.08.}


% \finding{Without providing any examples (i.e., shots) for the configuration validation query, \ourframework often reports false alarms or miss misconfigurations. However, by constructing a few examples in the validation query, we can effectively reduce wrongful predictions from \llms, and improve the \filelevel and \paramlevel \fonescore by up to 0.56 and 0.48, respectively. \label{finding:zeroshot}}

\finding{Without providing any examples (i.e., shots) for the configuration validation query, \llms often report false alarms or miss misconfigurations. For instance, \gptdavinci's F1-score plunges to as low as 0.08. \label{finding:zeroshot}}


\input{tables/finding2.tex}
%has both non-trivial false negatives and false positives. For instance, both GPT base models (Davinci-002 and Babbage-002) do not detect any \misconfig, and \gptdavinci's F1-scores plunge to as low as 0.08.

\noindent
Configuration shots play an important role in influencing the performance of LLMs. 
In scenarios where no \config shots are supplied,
    the performance of all \llms decreases considerably.  
\gptfour manages a parameter-level F1-score of 0.47,  
    while \gptturbo performs worse with a mere 0.24, 
    as illustrated in Table~\ref{tab:weekness}.
Without any shots, \davinci and \babbage cannot detect any misconfiguration in our dataset, we thus omitted them in Table~\ref{tab:weekness}.
This shows that shots are important towards improving \llms' inference performance for configuration validation, as they were in other learning tasks~\cite{brown:arxiv:20}.
% , \sam{this is because...}. 

% In Table~\ref{tab:weekness}, we present the overall evaluation results of \llms when no validation examples (shots) generated from \ourframework were provided.
% We can see that the performance of all \llms decrease considerably. 
% In particular, comparing Table~\ref{tab:weekness} to Table~\ref{tab:overview}, the average \fonescore of the top-three \llms has decreased by \fillnum{XXX\%-XXX\%} at \filelevel, and decreased by \fillnum{XXX\%-XXX\%} at \paramlevel. 
% Without any shots, \davinci and \babbage cannot detect any misconfiguration in our dataset, we thus omitted them in Table~\ref{tab:weekness}.
% This shows that shots are important towards improving \llms' inference performance for configuration validation task, as they were in other learning tasks~\cite{brown:arxiv:20}, \sam{this is because...}. 
% From Table~\ref{tab:weekness} to Table~\ref{tab:overview}, we also observe drops in \recall, but increases in \precision across \llms. This observation indicates that the models are reporting less false alarms, but missing more actual misconfigurations under zero-shot scenario.


\para{Implication.} 
Generating and providing configuration validation examples along with the validation query can improve off-the-shelf \llms' misconfiguration detection effectiveness.
We should acquire deeper understanding on how to construct better configuration file shots from real-world or historical misconfigurations to better adopt \llms as practical configuration validators. 

%Configuration shots play an important role in influencing the performance of LLMs. 
%In scenarios where no \config shots are supplied, 
%    \gptturbo manages a parameter-level F1-score of 0.24,  
%    while \gptdavinci performs worse with a mere 0.08, as illustrated in Table~\ref{tab:weekness}.
%The parameter-level precision of these two models is 0.16 and 0.08, respectively. 
%This indicates a significant volume of false positives when detecting \misconfig. 
%As for false negatives, \gptdavinci has a recall of 0.09, 
%    suggesting a non-trivial presence of undetected \misconfigs.
%Notably, the \gptfour model, though being slower and more expensive to use, 
%    distinguishes itself in \config validation tasks. 
%Despite being over 20 times more expensive than \gptturbo~\cite{openaipricing},
%    even in the absence of \config shots, 
%    it delivers a parameter-level F1-score of 0.47, 
%    showing its great generalization capabilities.
%This suggests that, when budget allows, 
%    investing in a more advanced model such as \gptfour 
%    can yield superior results, 
%    emphasizing the critical role of model selection again.

\finding{X\% reasons provided by the \llms are not comprehensible or not relevant to the misconfigurations. }
\yf{@Sam @Xinyu. Waiting for the result.
show one or two examples here, and try to explain why they reason badly for the case.}

% ==============================================
\subsection{All About Shots}
\label{sec:eval:shot}
% \ourframework's effectiveness is greatly influenced by combination of 
%     the ValidConfig and Misconfig shots.
Following the implications of Finding~\ref{finding:zeroshot}, 
    we conduct a series of experiments 
    to study how the configuration validation effectiveness 
    changes with different shot combinations.

We evaluate six $N$-shot learning settings, where $N$ can be 0 to 5. 
Under each setting, we use \ourframework to generate different combinations 
    of shots drawn from the \validconfig and \misconf database in the evaluated projects (\S\ref{sec:meth}).
For example, to evaluate \gptturbo on \hcommon in the $2$-shot setting, four experiments will be performed: (1) two \validconfig shots; (2) one \validconfig shot plus one \misconf shot; (3) two \misconf shots, drawn from the \hcommon's shot database. 
In total, we experiment with 21 shot combinations per project per \llm. 
To control computation cost, we limit this part of our evaluation 
    to two \llms (\gptturbo and \gptdavinci) on three systems 
    (\hbase, \hcommon, \alluxio).


\phantomsection\finding{It is essential to include both \validconfig  
    and \misconf in the shots;
    otherwise, the \llms may become biased.
    Both \gptturbo and \gptdavinci achieve their highest F1-scores 
    when provided with one \validconfig and three \misconf shots.}
\label{finding:bothshots}

% Following the implications of Finding~\ref{finding:zeroshot}, we study how the configuration validation effectiveness of \llms changes with different shot combinations in few-shot learning setting. 
% We evaluate 21 $N$-shot learning settings, where $N$ can be 0 to 5. 
% Under each setting, We use \ourframework to generate different combinations of configuration file shots drawn from the \validconfig and \misconf shot database in the evaluated projects (\S\ref{sec:meth}).
% For example, to evaluate \gptturbo on \hcommon in the $2$-shot setting, we in total perform 4 experiments: (1) two \validconfig shots; (2) one \validconfig shot plus one \misconf shot; (3) two \misconf shots, drawn from the \hcommon shot pool. 
% In total, we experiment with \fillnum{XXX} shot combinations per project per \llm. 


\phantomsection\finding{However, the labeled \misconfig, 
    despite being significantly lacking in practice, 
    is more crucial to validation effectiveness of \ourframework than \validconfig.
    Relying solely on \validconfig, 
    \gptturbo does not achieve parameter-level F1-scores higher than 0.25.
    However, when \misconf shots are introduced, 
        \gptturbo's F1-scores consistently exceed above 0.35.}
\label{finding:misconfig}
    
% Guidance \misconf in the form of ``shots'' are foundational to \ourframework's effectiveness.}
As shown in Figure~\ref{fig:heatmapcodex}-\ref{fig:heatmapturbo}, 
    \misconf shots allow \ourframework to more effectively identify 
    patterns and attributes commonly associated with \misconfigs, 
    surpassing the capabilities offered by \validconfig. 
In the absence of labeled \misconf, 
    the ability of \ourframework becomes limited. 
With \gptdavinci, \ourframework only gets an F1-score of approximately 0.2 
    (as denoted by the first column of the heat map), 
    when only using \validconfig shots in the prompt. 

Only relying on labeled \misconf can also inadvertently bias the model,
    since the input text distribution significantly impacts 
    the performance of \llms~\cite{min:arxiv:22}.
In our evaluation, there is not a direct correlation 
    between the number of \validconfig shots and the reduction in FP or FN cases
    e.g., the FP reduction rate is directly proportional 
    to the number of \validconfig shots. 
However, introducing the \validconfig shot does reduce FP cases for \gptdavinci
    and FN cases for \gptturbo.
This indicates that, by incorporating both \misconf and \validconfig, 
    \ourframework gains a more balanced perspective. 
    % enabling it to discern between \misconfigs and valid \configs 
    % that might superficially resemble an erroneous pattern. 

\input{figs/heatmap.tex}

% \phantomsection\finding{It is challenging, but also crucially important, 
%         to achieve a balanced integration of \validconfig  
%     and \misconf in few-shot learning. 
%     Otherwise, the \llms will become biased.
%     Both \gptturbo and \gptdavinci achieve their highest F1 scores 
%     when provided with one \validconfig and three \misconf shots.}
% \label{finding:5}

% Due to the prohibitive cost and strict rate limit associated with \gptfour, 
%     the exhaustive experiment of different shot combinations for \gptfour was not conducted.
% Instead, we test it with only one setting, 
%     i.e., one \validconfig and three \misconf shots,
%     which is the same as the best setting for \gptturbo and \gptdavinci,
%     since we believe that this setting is likely to be effective for \gptfour. 
% If not specified, the following experiments are also done with this setting.
% Note that, though \gptfour has already performed quite well, 
%     it may achieve better results with alternative shot settings.

The Finding \hyperref[finding:bothshots]{4} and \hyperref[finding:misconfig]{5} emphasize the importance of a holistic prompt examples 
    including both \validconfig and \misconf, 
    since over-relying on just one type of shot might compromise \ourframework.

% \jie{The original three findings convey the same message. I've merged them into one. Please reduce the redundancy in the paragraphs above.}

% \finding{The effectiveness of \ourframework is greatly influenced by the shot file selection strategy. Both Diff-Category and Similarity selection individually contribute to effectiveness. However, the hybrid 'Diff-Category + Similarity' method stands out as the most effective.}

% \finding{\tianyin{I don't understand this finding} Both Diff-Category and Similarity shot file selection strategies individually contribute to \ourframework's effectiveness, and the hybrid of these two methods stands out as the most effective.}

% \jie{Just providing an example here: You need to summarize/rephrase the findings to a more high-level/abstract finding. E.g., 

% high-level finding: the selection of in-context examples is important.

% Sub-findings: 1) Diversity; 2) Similarity/Relevance; 3) ...}

% \jie{Related works on in-context example selection: \url{https://aclanthology.org/2022.deelio-1.10/}, \url{https://openreview.net/forum?id=qY1hlv7gwg}}

% \finding{When the shot is selected from the same project, \llms demonstrate considerably better effectiveness than others scenarios.}

\phantomsection\finding{Leveraging configuration data from different projects as shots, 
    especially when the target project's data is unavailable, 
    showcases the transferability of \ourframework.
    For instance, when using \configs from other projects as shots for \hcommon's validation, 
    \ourframework maintains acceptable effectiveness, 
    achieving a parameter-level F1-score up to 0.44.}
    \label{finding:transfer}
% \yf{I found this finding is awkward. It is lower than the zero-shot..}
In scenarios where accessing configuration data 
    from a specific project might be challening,
    \ourframework's transferability becomes crucial.
To evaluate this transferability,
    the experiment is designed to use the shot files 
    from projects that are different from the target.


The results in Table~\ref{tab:cross-project shot} emphasizes 
    a critical aspect of \ourframework: 
    the ability to apply knowledge across different systems.  
While there's a decline in effectiveness 
    when compared to using \hcommon's native \configs as shots, 
    \ourframework still manages to achieve acceptable F1-scores. 
For models like \gptturbo and \gptdavinci, 
    their efficacy surpasses that of zero-shot learning 
    (as shown in Table~\ref{tab:weekness}). 
In contrast, for \gptfour, regardless of the project, 
    its performance consistently falls short of 
    its zero-shot learning (F1-score 0.53).
This observation hints that, for advanced models like \gptfour,
    it is better to not use shots than 
    using shots from other projects,
    as the latter could introduce more biases. 

    \input{tables/cross-system.tex}
    % \jie{this explanation seems not good. You can simply say ``for most models, the performance is better than 0-shot''. BTW, the meaning of gray may need to be explained, and how the transferability is conducted is not explained, e.g., which transfer to which? (the presentation of the results is quite confusing to me)}
% In the rapidly evolving cloud landscape, it's essential for tools like \ourframework 
%     to not just excel within a singular project 
%     but also demonstrate adaptability when introduced to others.

% \xinyu{The reason to do provide the shot from hadoop and hbase to alluxio in our experiment:
% 1) both hadoop and hbase is from apache and share the same config api, while the alluxio are quite different.
% 2) both hadoop and hbase is using the xml format for config file, while the alluxio is using the properties format that is in pure key-value pair.
% 3) the first version of hadoop is released in 2007 and hbase is in 2008 while the alluxio is in 2016.
% 4) the average G-hits of Hadoop's parameters is 1767, hbase is 1752, while the alluxio is 86.

% We want to show that even though the target project is quite different from the shot project (config file format is diff, api is diff, belong to diff org, quite new), \ourframework can still achieve a high level of effectiveness.}

% \finding{Leveraging the probabilities of tokens to establish the threshold has proven advantageous.

% \finding{Providing detailed descriptions of configuration parameters seemed to impede rather than improve the effectiveness of LLMs.}

% \jie{Like what we discussed before, this may due to the variance or prompt design. A good finding needs to be generalized and not specific to a model and a prompt.}

% \sam{Because some people might be skeptical on whether some design choice findings can be generalized, spend some text sharing your experience on how to deal with these design complexity, and providing more implications are perhaps more useful to other system practitioners.}


\finding{The effectiveness (parameter-level F1-score) of \fw is improved by up to 37.0\%/69.5\% 
if provided \misconf shot contains \misconfig that share the same category/sub-category as the \misconfig in the to-be-validated 
\misconf file.}
\input{tables/relevant-shot.tex}

\subsection{When Do Things Go South}
\label{sec:eval:bias}
% \subsection{Effect of Task Difficulty}

\finding{\ourframework excels in pinpointing \misconfigs in most sub-categories (12 out of 15), 
    but does not show the same proficiency for Dependency and Version categories.}

Table~\ref{tab:result_category} shows the effectiveness of 
    \ourframework in identifying various types of \misconfigs.
A closer inspection reveals that for the sub-categories: 
    Control, Value Relationship, and Parameter Change, 
    \ourframework's F1-scores do not surpass the 0.30 in most cases.
This performance is significantly lower than other categories.
Notably, only \gptfour achieves a slightly better F1-score of 0.46 
    for the Value Relationship, 
    but this is also significantly lower than its other results.
% To give equal weight to each \config in the same sub-category regardless of its project,
Note that, to treat \configs in the same category 
    equally regardless of its project, 
    we calculate the Micro F1-score for the average.

The difference in performance can be attributed to 
    the inherent nature of the \misconfigs themselves. 
Sub-categories like Syntax and Range are more universal 
    and are areas where \llms have learned extensive knowledge from diverse sources. 
% These types of misconfigurations are akin to general computer science knowledge, 
%     which even a person with basic training can detect.
On the other hand, Dependency and Version categories are more project-specific. 
They are closely linked to the specific details of individual projects, 
    making them harder for models, 
    without extensive training on that project's data.
While general computer science knowledge might suffice to spot Syntax or Range errors,
    detecting \misconfigs related to dependencies or versioning would likely 
    require the expertise of the model deeply familiar with the project.
This distinction underscores the challenges faced by \ourframework 
    and highlights the importance of context-specific knowledge in \config validation.
\yf{@Xinyu, case study here.}
% \yf{Possible reasons why they are poor: 1. Complexity and Ambiguity; 2. Lack of training data.
% Consider comparing these with human's validation ability for these categories;
% and also case study here.}

% *use a vinn figure here for three models to see the difference on different types or parameters.
% \yf{@Xinyu, calculate avg for these three models.}
% \yf{Here the F1 is micro F1 since the different categories have different number of parameters.}
\input{tables/result_over_category.tex}


% \yf{Need to emphasize that we use the 1-3 setting for the experiment somewhere.}
\finding{As the number of parameters increases in the \config file under test, the effectiveness of \ourframework decreases.}
As shown in Figure~\ref{fig:numparam}, this decline in \ourframework's performance 
    can be attributed to a potential information overload for \llms. 
As the complexity of the \config file grows, 
    the potential combinations and dependencies 
    between \config parameters also grow exponentially. 
    the model may struggle to process and understand the complex relationships 
    between the increasing number of parameters.
For instance, when the number of parameters jumps from 8 to 16, 
the performance of \ourframework begins to deteriorate severely.
This trend mirrors the challenges faced in other domains 
    where models are presented with an abundance of information, 
    often leading to decreased performance 
    as essential data become obscured amidst the surrounding noise.
% \yf{@Jie, are there any references to support my point? If there is no reference, I will revise the last sentence.}
% \jie{I feel this is something intuitive -- as the difficult increases, performance decreases.}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/numParam.pdf}
    \caption{Effectiveness of GPT-3.5-turbo across different number of parameters in the \config file under test.}
    \label{fig:numparam}
\end{figure}


\subsection{Echoes from Afar}
% External Echoes
% LLM Catalysts
% External LLM Levers

\finding{Upon evaluation with the \validconfig dataset, 
    \ourframework leans more towards parameters that have higher G-hits, 
    indicating a direct correlation between a parameter's popularity in Google searches 
    and the likelihood of the LLM addressing it.}

\textbf{G-hits}: A metric quantifying the prevalence of a specific keyword based on its appearances in Google search results. Specifically, G-hits index denotes the number of exact-match search results returned by Google for a keyword. 

As demonstrated in Figure~\ref{fig:Ghits Correct}, parameters within the \config 
    under examination are ranked based on their corresponding G-hits index. 
For the \validconfig dataset, we counted the frequency with which \ourframework 
    identifies each ranked parameter. 
Specifically, we recorded how often \ourframework targets the parameter ranked first by G-hits, 
    the parameter ranked second, and so forth. 
If \ourframework marks multiple parameters as \misconfigs when testing a single \config file, 
    frequency will be distributed evenly across all of them.
Intriguingly, the distribution reveals a clear skewness towards parameters 
    with higher G-hits rankings. 
This trend can be attributed to the nature of the training data for \llms. 
Training data is often sourced from publicly 
    accessible domains (e.g., Common Crawl~\cite{commoncrawl}), 
    easily accessible by search engine like Google, 
    which significantly influences \llms behavior. 
Popular topics or parameters are more likely embedded deeply into 
    the model's knowledge due to their prevalence in the training data.

\input{figs/ghit.tex}

% Ranked with G-hints, $8^{th}$ parameter is pinpointed 23 times. $1^{st}$ parameter is pinpointed 73 times.


% \finding{Within invalid \conffiles, \llms demonstrate enhanced accuracy in detecting invalid value of parameters with higher G-hints.}

\finding{When evaluated using the labeled \misconf dataset, 
    \ourframework exhibits greater precision in identifying incorrect values 
    for parameters that have higher G-hints.}
In the evaluation of the labeled \misconf dataset, 
    we observe a trend: 
parameters with higher G-hints, indicating their prevalence in search results, 
    are more accurately identified by \ourframework when they have incorrect values. 
Specifically, the median G-hits value 
    for correctly detected misconfigurations 
    is notably higher than that for misconfigurations 
    that \ourframework fails to identify. 

% \jie{The above two findings need to be combined to one finding}

% \yf{Box plot please. @Xinyu}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.75\linewidth]{figs/box_figure.pdf}
    \vspace{-0.2cm}
    \caption{Distribution of G-hits for misconfigured parameters. 
    Left box represents G-hits distribution of parameters correctly detected, 
    while right box indicates the distribution of parameters that are failed to detect.}
    \label{fig:Ghits Wrong}
\end{figure}

% \input{tables/strategy}

% \finding{Bias on the parameter's non-default value: X\% false positives generated by LLMs can be attributed to X, i.e., LLMs tend to pinpoint parameters whose values deviate from their default values more frequently.}

% \finding{Bias on new projects beyond the training dataset: LLMs exhibited noticeably reduced effectiveness on new projects that they are not trained on. } 

% \jie{Haven't seen the results yet. Need to provide some quantitative analysis on the data/corpus to support the findings.}


% \finding{\llms sometimes pinpoint parameters even if they are set to their default values.}
\finding{Despite LLMs being aware of default parameter values, they occasionally flag these default settings as misconfigurations during detection tasks.}
\yf{@Xinyu, calculate percentage for the default value that LLMs know.}

We query LLMs to determine their awareness of default parameter values. 
For each LLM, we calculate the percentage of default values they correctly answer. 
\gptfour, \gptturbo, and \gptdavinci are aware of the \yf{XX, XX, XX} default values respectively.
The goal is to ascertain if \fw could correctly identify 
    these default settings without flagging them as misconfigurations. 
Surprisingly, even with the high percentage of their knowledge 
    about the default value of some parameters, 
    LLMs still occasionally misinterpreted these default values.
As illustrated in Table~\ref{tab:default_v}, 
    there isn't a consistent pattern between 
    the mis-detection of default values and non-default values; 
    both can be erroneously flagged by LLMs.

% \yf{I think the avg is also a macro avg for percentage? @Xinyu}
% \yf{Case study?}
 \input{tables/default_v.tex}
% \input{tables/pinpoint_default.tex}










==> sections/futurework.tex <==
\section{Future Work}
\label{sec:futurework}



==> sections/limitation.tex <==
\section{Limitations and Future Work}

\tianyin{Here we should discuss what we should have done but didn't do.
It is more or less apologies.}

==> sections/numQuery.tex <==

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.3\linewidth]{figs/numQuery.pdf}
    \caption{Effectiveness of voting mechanism of \fw and the number of queries.}
    \label{fig:numQuery}
\end{figure}
\finding{Compared to only provide answer by querying once, the voting mechanism of \fw via multple queries can improve the para-level f-1 score by 3\%.}

The result here is not so good, the main reason is that we set the temperature to a low value (0.2) to make the model more conservative.
I suggest to put the data to S3 instead of a new finding.
We can also claim the Finding3 shows the reason provided by LLms are not always comprehensible so that via multiple queries we can get multiply reasons to avoid such issue.


==> tables/change-format.tex <==
\begin{table}[ht]
  \footnotesize
    \setlength{\tabcolsep}{4.6pt}
    \centering
    \begin{tabular}{c|cccc|ccc}
      \toprule
      \multirow{2}{*}{\bf \# Shots} & \multicolumn{4}{c}{\bf \% CVC} & \multicolumn{3}{c}{\bf \% F1-Score} \\
      {} & {XML} & {KV} & {Ratio} & & {XML} & {KV} & {Ratio} \\
      \midrule
      0 & 6.81 \% & 00.00\% & 0.00 & & 13.33\% & 00.00\% & 0.00 \\
      1 & 53.41\% & 35.84\% & 0.67 & & 63.49\% & 42.77\% & 0.67 \\
      2 & 64.87\% & 54.48\% & 0.84 & & 71.13\% & 61.32\% & 0.86 \\
      3 & 72.76\% & 59.14\% & 0.81 & & 77.13\% & 65.38\% & 0.85 \\
      4 & \cellcolor{LightGray} 75.27\% & 64.87\% & 0.86 & & \cellcolor{LightGray} 78.58\% & 69.58\% & 0.90 \\
      5 & 74.55\% & 64.87\% & 0.87 & & 78.13\% & 69.85\% & 0.89 \\
      6 & -       & 71.33\% & -    & & -       & 74.53\% & -    \\
      7 & -       & \cellcolor{LightGray} 72.76\% & -    & & -       & \cellcolor{LightGray} 76.17\% & -    \\
      8 & -       & 66.31\% & -    & & -       & 69.55\% & -    \\
      9 & -       & 64.16\% & -    & & -       & 68.32\% & -    \\
      \midrule
      $Avg$ &     &         & 0.68 & &         &         & 0.70 \\
      \bottomrule
      \end{tabular}
      \caption{Effectiveness of \itcodedavinci in misconfiguration detection for different format of configuration files.}
      \label{tab:results:change-format}
\end{table}


==> tables/cross-system-v2.tex <==
\begin{table*}[!htb]
    \setlength{\tabcolsep}{3.5pt}
    \tiny
    \centering
    \begin{tabular}{l|l|llll|llll|llll|llll|llll|ll}
        \toprule
        \multirow{3}{*}{\bf Models}                    & \multicolumn{8}{c}{\bf F1-score}   & \multicolumn{8}{c}{\bf Precision}    & \multicolumn{7}{c}{\bf Recall}   \\
         & \multicolumn{4}{c}{File Level} & \multicolumn{3}{c}{Param Level} & & \multicolumn{4}{c}{File Level} & \multicolumn{3}{c}{Param Level} & & \multicolumn{4}{c}{File Level} & \multicolumn{3}{c}{Param Level} \\
         \cline{2-4}
         \cline{6-8}
         \cline{10-12}
         \cline{14-16}
         \cline{18-20}
         \cline{22-24}
         & HA. & HB. & & & HA. & HB. & & & HA. & HB. &  & & HA. & HB. &  & & HA. & HB. &  & & HA. & HB. &  \\
         \midrule
         {GPT-4} & 0.80 & 0.72 & & & 0.64 & 0.42\\
        {GPT-3.5-turbo} &  0.74 & 0.72 && & 0.52 & 0.30\\
        {Code-Davinci-002} &  0.74 & 0.73 & & &  0.59 & 0.47\\
      \bottomrule
      \end{tabular}
      \caption{Effectiveness of \fw on \hcommon with shot files from either \hbase}
      \label{tab:cross-system-v2}
\end{table*}


==> tables/default_v.tex <==
\begin{table*}[!htb]
    \setlength{\tabcolsep}{3pt}
    \scriptsize
    \caption{Percentage of samples where LLMs identify default and valid (non-default) values as invalid.}
    \vspace{-10pt}
    \centering
    \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
        \toprule
        \multirow{3}{*}{\bf Models}     & \multicolumn{2}{c}{\bf HC.} &  & \multicolumn{2}{c}{\bf HB.}  &  & \multicolumn{2}{c}{\bf AL.} && \multicolumn{2}{c}{\bf HD.} && \multicolumn{2}{c}{\bf YA.}&& \multicolumn{2}{c}{\bf ZK.} & & \multicolumn{2}{c}{\bf Avg.}   \\
        %  \cline{2-3}
        %  \cline{5-6}
        %  \cline{8-9}
        %  \cline{11-12}
        %  \cline{14-15}
        %  \cline{17-18}
        %  \cline{20-21}
        %  \cline{23-24}
         &Def. & N.D. & &  Def. & N.D. &&  Def. & N.D. & &  Def. & N.D. &&  Def. & N.D.&&  Def. & N.D. &&  Def. & N.D. \\
         \midrule
         {GPT-4} &4.4\%&7.6\%&&10.7\%&4.7\%&&6.7\%&6.2\%&&5.8\%&5.9\%&&5.9\%&8.4\%&&18.1\%&10.8\% & & \cellcolor{Gray}8.6\%&7.3\%\\ 
        {GPT-3.5-turbo} &6.3\%&5.1\%&&4.7\%&3.7\%&&9.0\%&9.5\%&&4.7\%&4.7\%&&7.0\%&7.5\%&&14.0\%&8.5\%&&\cellcolor{Gray}7.6\%&6.5\%&\\ 
        {Code-Davinci-002}&3.6\%&5.4\%&&3.6\%&4.2\%&&2.8\%&5.3\%&&4.3\%&5.7\%&&5.4\%&7.5\%&&10.0\%&6.9\%&& 4.9\%&\cellcolor{Gray}5.8\%\\ 
      \bottomrule
      \end{tabular}
      \label{tab:default_v}
\end{table*}


==> tables/diff-model.tex <==
\begin{table*}[ht]
    \setlength{\tabcolsep}{8pt}
    \centering
    \begin{tabular}{ll|rrrrr|rrrr}
        \toprule
        \multirow{2}{*}{\bf } & \multirow{2}{*}{\bf } & \multicolumn{4}{c}{\bf \codedavinci} & & \multicolumn{4}{c}{\bf \textdavinci} \\
        \multirow{5}{*}{\bf 0-shot} & {} & {\hcommon} & {\hbase} & {\alluxio} & {$avg$} & & {\hcommon} & {\hbase} & {\alluxio} & {$avg$} \\ 
        {} & {\% Precision} & \zeroHCommonCdPrecision & \zeroHBaseCdPrecision & \zeroAlluxioCdPrecision & \zeroAvgCdPrecision & & \zeroHCommonTdPrecision & \zeroHBaseTdPrecision & \zeroAlluxioTdPrecision & \zeroAvgTdPrecision \\
        {} & {\% CVC}    & \zeroHCommonCdCVC & \zeroHBaseCdCVC & \zeroAlluxioCdCVC & \zeroAvgCdCVC & & \zeroHCommonTdCVC & \zeroHBaseTdCVC & \zeroAlluxioTdCVC & \zeroAvgTdCVC \\ 
        \midrule
        \multirow{5}{*}{\bf 1-shot} & {} & {\hcommon} & {\hbase} & {\alluxio} & {$avg$} & & {\hcommon} & {\hbase} & {\alluxio} & {$avg$} \\ 
        {} & {Precision} & \oneHCommonCdPrecision & \oneHBaseCdPrecision & \oneAlluxioCdPrecision & \oneAvgCdPrecision & & \oneHCommonTdPrecision & \oneHBaseTdPrecision & \oneAlluxioTdPrecision & \oneAvgTdPrecision \\ 
        {} & {\% CVC}   &  \oneHCommonCdCVC & \oneHBaseCdCVC & \oneAlluxioCdCVC & \oneAvgCdCVC & & \oneHCommonTdCVC & \oneHBaseTdCVC & \oneAlluxioTdCVC & \oneAvgTdCVC \\ 
        \midrule
        \multirow{5}{*}{\bf 2-shot} & {} & {\hcommon} & {\hbase} & {\alluxio} & {$avg$} & & {\hcommon} & {\hbase} & {\alluxio} & {$avg$} \\ 
        {} & {\% Precision} & \twoHCommonCdPrecision & \twoHBaseCdPrecision & \twoAlluxioCdPrecision & \twoAvgCdPrecision & & \twoHCommonTdPrecision & \twoHBaseTdPrecision & \twoAlluxioTdPrecision & \twoAvgTdPrecision \\
        {} & {\% CVC}    & \twoHCommonCdCVC & \twoHBaseCdCVC & \twoAlluxioCdCVC & \twoAvgCdCVC & & \twoHCommonTdCVC & \twoHBaseTdCVC & \twoAlluxioTdCVC & \twoAvgTdCVC \\ 
      \bottomrule
      \end{tabular}
      \caption{Comparison between different Large Language Models in misconfiguration detection.}
      \label{tab:results:diff-model}
  \end{table*}

==> tables/diff-shot.tex <==
\begin{table*}[ht]
    \footnotesize
    \setlength{\tabcolsep}{3.5pt}
    \centering
    \begin{tabular}{c|ccccc|ccccc|cccc}
      \toprule
      \multirow{2}{*}{\bf \# Shots} & \multicolumn{5}{c}{\bf HCommon} & \multicolumn{5}{c}{\bf HBase} & \multicolumn{4}{c}{\bf Alluxio} \\
      {} & {\% CVC} & {\% Precision} & {\% Recall} & {\% F1} & {} & {\% CVC} & {\% Precision} & {\% Recall} & {\% F1} & {} & {\% CVC} & {\% Precision} & {\% Recall} & {\% F1} \\
      \midrule
      0 & \zeroHCommonCdCVC & \zeroHCommonCdPrecision & \zeroHCommonCdRecall & \zeroHCommonCdF & & \zeroHBaseCdCVC & \zeroHBaseCdPrecision & \zeroHBaseCdRecall & \zeroHBaseCdF & & \zeroAlluxioCdCVC & \zeroAlluxioCdPrecision & \zeroAlluxioCdRecall & \zeroAlluxioCdF \\ 
      1 & \oneHCommonCdCVC & \oneHCommonCdPrecision & \oneHCommonCdRecall & \oneHCommonCdF & & \oneHBaseCdCVC & \oneHBaseCdPrecision & \oneHBaseCdRecall & \oneHBaseCdF & & \oneAlluxioCdCVC & \oneAlluxioCdPrecision & \oneAlluxioCdRecall & \oneAlluxioCdF \\ 
      2 & \twoHCommonCdCVC & \twoHCommonCdPrecision & \twoHCommonCdRecall & \twoHCommonCdF & & \twoHBaseCdCVC & \twoHBaseCdPrecision & \twoHBaseCdRecall & \twoHBaseCdF & & \twoAlluxioCdCVC & \twoAlluxioCdPrecision & \twoAlluxioCdRecall & \twoAlluxioCdF \\ 
      3 & \threeHCommonCdCVC & \threeHCommonCdPrecision & \threeHCommonCdRecall & \threeHCommonCdF & & \threeHBaseCdCVC & \threeHBaseCdPrecision & \threeHBaseCdRecall & \threeHBaseCdF & & \threeAlluxioCdCVC & \threeAlluxioCdPrecision & \threeAlluxioCdRecall & \threeAlluxioCdF \\ 
      \rowcolor{LightGray}
      4 & \fourHCommonCdCVC & \fourHCommonCdPrecision & \fourHCommonCdRecall & \fourHCommonCdF & & \fourHBaseCdCVC & \fourHBaseCdPrecision & \fourHBaseCdRecall & \fourHBaseCdF & & \fourAlluxioCdCVC & \fourAlluxioCdPrecision & \fourAlluxioCdRecall & \fourAlluxioCdF \\ 
      5 & \fiveHCommonCdCVC & \fiveHCommonCdPrecision & \fiveHCommonCdRecall & \fiveHCommonCdF & & \fiveHBaseCdCVC & \fiveHBaseCdPrecision & \fiveHBaseCdRecall & \fiveHBaseCdF & & \fiveAlluxioCdCVC & \fiveAlluxioCdPrecision & \fiveAlluxioCdRecall & \fiveAlluxioCdF \\ 
      6 & \sixHCommonCdCVC & \sixHCommonCdPrecision & \sixHCommonCdRecall & \sixHCommonCdF & & \sixHBaseCdCVC & \sixHBaseCdPrecision & \sixHBaseCdRecall & \sixHBaseCdF & & \sixAlluxioCdCVC & \sixAlluxioCdPrecision & \sixAlluxioCdRecall & \sixAlluxioCdF \\ 
      7 & \sevenHCommonCdCVC & \sevenHCommonCdPrecision & \sevenHCommonCdRecall & \sevenHCommonCdF & & \sevenHBaseCdCVC & \sevenHBaseCdPrecision & \sevenHBaseCdRecall & \sevenHBaseCdF & & \sevenAlluxioCdCVC & \sevenAlluxioCdPrecision & \sevenAlluxioCdRecall & \sevenAlluxioCdF \\ 
      8 & \eightHCommonCdCVC & \eightHCommonCdPrecision & \eightHCommonCdRecall & \eightHCommonCdF & & \eightHBaseCdCVC & \eightHBaseCdPrecision & \eightHBaseCdRecall & \eightHBaseCdF & & \eightAlluxioCdCVC & \eightAlluxioCdPrecision & \eightAlluxioCdRecall & \eightAlluxioCdF \\ 
      9 & \nineHCommonCdCVC & \nineHCommonCdPrecision & \nineHCommonCdRecall & \nineHCommonCdF & & \nineHBaseCdCVC & \nineHBaseCdPrecision & \nineHBaseCdRecall & \nineHBaseCdF & & \nineAlluxioCdCVC & \nineAlluxioCdPrecision & \nineAlluxioCdRecall & \nineAlluxioCdF \\ 
      10 & \tenHCommonCdCVC & \tenHCommonCdPrecision & \tenHCommonCdRecall & \tenHCommonCdF & & \tenHBaseCdCVC & \tenHBaseCdPrecision & \tenHBaseCdRecall & \tenHBaseCdF & & \tenAlluxioCdCVC & \tenAlluxioCdPrecision & \tenAlluxioCdRecall & \tenAlluxioCdF \\ 
      \bottomrule
      \end{tabular}
      \caption{Effectiveness of \itcodedavinci in misconfiguration detection with different number of shots.}
      \label{tab:results:diff-shot}
\end{table*}

==> tables/finding.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \begin{tabular}{|p{8.65cm}|p{8.6cm}|}
        \hline
        {\bf Findings} & {\bf Implications} \\
        \hline
        {\textbf{F.1} Off-the-shelf (zero-shot), \codedavinci, \codecushman, \textdavinci can detect up to 45.74\%, 18.28\%, 1.55\% of misconfigurations, respectively.} & {\textbf{I.1}} \\
        \hline 
        {\textbf{F.2} In one-shot scenario, Code-Davinci-002, Code-Cushman-001, Text-Davinci-003 can detect up to 65.59\%, 11.47\%, 27.86\% of misconfigurations, respectively.} & {\textbf{I.2}} \\
        \hline
        {\textbf{F.3} Code-Davinci-002's performance increases approximately logarithmically by the number of shot. Its performance was saturated in four-shot and can detect up to 78.49\% of misconfigurations.} & {\textbf{I.3}} \\
        \hline
        {\textbf{F.4} The number of False Positive increases significantly from zero-shot to one-shot, and then decreases gradually with the increase of the number of shot.} & {\textbf{I.4}} \\
        \hline
        {\textbf{F.5} The basic model \codedavinci can detect more misconfigurations than the advanced fine-tuned model \textdavinci.} & {\textbf{I.5}} \\
        \hline
        {\textbf{F.6} When the shot contains the type of the ground truth misconfiguration parameter, model's performance improves 9.65\%.} & {\textbf{I.6}} \\
        \hline
        {\textbf{F.7} (cross-system shot) When shot contains samples from different systems, utilizing them in the model can also result in an improvement in performance compared to zero-shot learning, though the improvement is less significant than when using shot from the same system.} & {\textbf{I.7}} \\
        \hline
        {\textbf{F.8} (cross-system shot) When shot are from different systems, using the shot of the same format as the test configuration file can improve the performance of LLMs.} & {\textbf{I.8}} \\
        \hline
        {\textbf{F.9} Without metadata, Code-Davinci-002's performance saturates at five-shot and can detect up to 87.46\% of misconfigurations, which improves by 11.93\% compared to the scenario where the metadata is involved.} & {\textbf{I.9}} \\
        \hline
        {\textbf{F.10} Flattening xml configuration files to pure key-value pairs will decrease the performance of the model by 21\%.} & {\textbf{I.10}} \\
        \hline
        \end{tabular}
        \caption*{Table 1: Summary of findings and implications\label{finding}}
\end{table*}


==> tables/historical_issue.tex <==
\begin{table}[t]
    \footnotesize
    \setlength{\tabcolsep}{2.5pt}
    \centering
    \begin{tabular}{lcc}
      \toprule
      {\bf Root Cause} & {\bf \# Failures$\ \ $} & {\bf \# (\%) Detected by LLM} \\
      \midrule
      \rowcolor{LightGray}
      Misconfigurations                             & 21 & 9 (42.9\%) \\
      \rowcolor{VeryLightGray}
      $\quad \vdash$ Corrupt config files           & 1  & 0 ( 0.0\%) \\
      \rowcolor{VeryLightGray}
      $\quad \vdash$ Out-of-range values            & 5  & 3 (60.0\%) \\
      $\quad\quad \vdash$ Numeric                   & 1  & 0 ( 0.0\%) \\
      $\quad\quad \vdash$ Enum                      & 4  & 3 (75.0\%) \\
      \rowcolor{VeryLightGray}
      $\quad \vdash$ Value semantic errors          & 14 & 6 (42.9\%) \\
      $\quad\quad \vdash$ Permission mask/File path/URI/IP       & 8  & 6 (75.0\%)   \\
      $\quad\quad \vdash$ Blank space               & 3  & 0 ( 0.0\%) \\
      $\quad\quad \vdash$ Implicit                  & 3  & 0 ( 0.0\%) \\
      \rowcolor{VeryLightGray}
      $\quad \vdash$ Resource violations/ENV        & 1  & 0 ( 0.0\%) \\
      \hline
      \rowcolor{LightGray}
      Bugs exposed by valid config                  & 4  & 0 ( 0.0\%) \\
      \midrule
      Total                                         & 25 & 9 (36.0\%) \\
      \bottomrule
    \end{tabular}
    \vspace{-2.5pt}
    \caption{{\bf LLM effectiveness in detecting real-world configuration-induced
      failures of various root-cause types.}}
    \label{tab:error_type}
\end{table}

==> tables/no_metadata.tex <==
\begin{table}[h]
    \setlength{\tabcolsep}{8.5pt}
    \centering
    \begin{tabular}{l|cccccc}
      \toprule
      {\# Shots}  & \multicolumn{2}{c}{HCommon}  & \multicolumn{2}{c}{HBase}  & \multicolumn{2}{c}{Alluxio} \\
      {} & {WM} & {NM} & {WM} & {NM} & {WM} & {NM} \\
      \midrule
      {0-shot}  & {38.71} & {37.63} & {45.74} & {55.81} & {27.60} & {36.20} \\
      {1-shot}  & {65.59} & {63.80} & {62.40} & {72.87} & {45.16} & {53.76} \\
      {2-shot}  & {70.25} & {69.53} & {68.99} & {75.58} & {51.25} & {55.91} \\
      {3-shot}  & {78.14} & {77.42} & {70.54} & {77.52} & {58.42} & {63.44} \\
      {4-shot}  & {78.49} & {82.08} & {72.48} & {77.91} & {63.08} & {65.23} \\
      {5-shot}  & {78.14} & {87.46} & {71.71} & {79.84} & {63.08} & {66.67} \\
      {6-shot}  & {N.A.}  & {89.25} & {N.A.}  & {78.68} & {63.44} & {69.89} \\
      {7-shot}  & {N.A.}  & {89.61} & {N.A.}  & {82.95} & {64.16} & {71.68} \\
      {8-shot}  & {N.A.}  & {91.76} & {N.A.}  & {81.78} & {64.52} & {72.40} \\
      {9-shot}  & {N.A.}  & {91.04} & {N.A.}  & {85.27} & {59.86} & {72.04} \\
      {10-shot} & {N.A.}  & {N.A.}  & {N.A.}  & {N.A.}  & {59.50} & {71.68} \\
      {11-shot} & {N.A.}  & {N.A.}  & {N.A.}  & {N.A.}  & {N.A.}  & {72.40} \\
      {12-shot} & {N.A.}  & {N.A.}  & {N.A.}  & {N.A.}  & {N.A.}  & {70.25} \\
      {13-shot} & {N.A.}  & {N.A.}  & {N.A.}  & {N.A.}  & {N.A.}  & {71.33} \\
      {14-shot} & {N.A.}  & {N.A.}  & {N.A.}  & {N.A.}  & {N.A.}  & {73.84} \\
      {15-shot} & {N.A.}  & {N.A.}  & {N.A.}  & {N.A.}  & {N.A.}  & {72.04} \\
      \bottomrule
      \end{tabular}
      \caption{The performance of \textit{Code-Davinci-002} affected by the metadata.}
      \label{tab:results:no_metadata}
  \end{table}


==> tables/notation.tex <==
\begin{table}
    \scriptsize
    \setlength{\tabcolsep}{3pt}
    \centering
    \begin{tabular}{lp{7.35cm}}
      \toprule
      {\bf Notation} & {\bf Description} \\
      \midrule
      \# TP    & The number of queries that correctly detect misconfigurations.\\
      \# FP    & The number of queries that falsely detect correct configuration parameters.\\
      \% CVC   & Short for Correct Voting Candidates. See Section\ref{sec:meth:vm} for detailed explanation.\\
      \% Once  & The percentage that correct pinpoint appears once among the ten queries.\\ 
      \% Major & The percentage that correct pinpoint appears more than half of the time among the ten queries.\\ 
      \% Every & The percentage that correct pinpoint appears every time among the ten queries.\\ 
      \bottomrule
      \end{tabular}
      \caption{Notations used in the paper and their descriptions.}
      \label{tab:notation}
  \end{table}


==> tables/pinpoint_default.tex <==
\begin{table*}[!htb]
    \tiny
    \setlength{\tabcolsep}{5pt}
    \centering
    \begin{tabular}{lllllllllllll}
        \toprule
        \multirow{2}{*}{\bf Project}  & \multirow{2}{*}{\bf \#CS} & \multirow{2}{*}{\bf \#WS} & \multirow{2}{*}{\bf SSM}  & \multicolumn{2}{c}{\gptdavinci} & & \multicolumn{2}{c}{\gptturbo} & &  \multicolumn{2}{c}{\gptfour}  \\
        \cline{5-6}
        \cline{8-9}
        \cline{11-12}
        & & & & Valid & Invalid & & Valid & Invalid & & Valid & Invalid \\
        \midrule
HCommon & 0 & 0 & random & 3/64 & 8/64 & & 22/64 & 31/64 & &  & \\
HCommon & 1 & 0 & random & 0/64 & 2/64 & & & & &  & \\
HCommon & 2 & 0 & random & 0/64 & 0/64 & & & & &  & \\
HCommon & 3 & 0 & random & 0/64 & 0/64 & & & & &  & \\
HCommon & 4 & 0 & random & 0/64 & 0/64 & & & & &  & \\
HCommon & 5 & 0 & random & 0/64 & 0/64 & & & & &  & \\
HCommon & 0 & 1 & random & 8/64 & 12/64 & & & & &  & \\
HCommon & 1 & 1 & random & 11/64 & 6/64 & & & & &  & \\
HCommon & 2 & 1 & random & 4/64 & 1/64 & & & & &  & \\
HCommon & 3 & 1 & random & 1/64 & 1/64 & & & & &  & \\
HCommon & 4 & 1 & random & 0/64 & 1/64 & & & & &  & \\
HCommon & 0 & 2 & random & 18/64 & 10/64 & & & & &  & \\
HCommon & 1 & 2 & random & 18/64 & 8/64 & & & & &  & \\
HCommon & 2 & 2 & random & 1/64 & 3/64 & & & & &  & \\
HCommon & 3 & 2 & random & 0/64 & 5/64 & & & & &  & \\
HCommon & 0 & 3 & random & 23/64 & 7/64 & & & & &  & \\
HCommon & 1 & 3 & random & 14/64 & 7/64 & & & & &  & \\
HCommon & 2 & 3 & random & 3/64 & 6/64 & & 27/64 & 14/64& &  & \\
HCommon & 0 & 4 & random & 23/64 & 10/64 & & & & &  & \\
HCommon & 1 & 4 & random & 17/64 & 10/64 & & 18/64 & 9/64 & &  & \\
HCommon & 0 & 5 & random & 27/64 & 15/64 & & & & &  & \\        
HBase & 0 & 0 & random & 6/50 & 4/50 & & & & &  & \\
HBase & 1 & 0 & random & 4/50 & 15/50 & & & & &  & \\
HBase & 2 & 0 & random & 6/50 & 2/50 & & & & &  & \\
HBase & 3 & 0 & random & 12/50 & 7/50 & & & & &  & \\
HBase & 4 & 0 & random & 6/50 & 6/50 & & & & &  & \\
HBase & 5 & 0 & random & 2/50 & 4/50 & & & & &  & \\
HBase & 0 & 1 & random & 3/50 & 9/50 & & & & &  & \\
HBase & 1 & 1 & random & 11/50 & 8/50 & & & & &  & \\
HBase & 2 & 1 & random & 13/50 & 5/50 & & & & &  & \\
HBase & 3 & 1 & random & 5/50 & 3/50 & & & & &  & \\
HBase & 4 & 1 & random & 5/50 & 6/50 & & & & &  & \\
HBase & 0 & 2 & random & 7/50 & 9/50 & & & & &  & \\
HBase & 1 & 2 & random & 10/50 & 4/50 & & & & &  & \\
HBase & 2 & 2 & random & 9/50 & 2/50 & & & & &  & \\
HBase & 3 & 2 & random & 6/50 & 4/50 & & & & &  & \\
HBase & 0 & 3 & random & 4/50 & 4/50 & & & & &  & \\
HBase & 1 & 3 & random & 10/50 & 7/50 & & & & &  & \\
HBase & 2 & 3 & random & 8/50 & 9/50 & & & & &  & \\
HBase & 0 & 4 & random & 2/50 & 2/50 & & & & &  & \\
HBase & 1 & 4 & random & 6/50 & 3/50 & & 4/50& 7/50& &  & \\
HBase & 0 & 5 & random & 5/50 & 2/50 & & & & &  & \\
Alluxio & 0 & 0 & random & 0/54 & 0/54 & & & & &  & \\
Alluxio & 1 & 0 & random & 4/54 & 8/54 & & & & &  & \\
Alluxio & 2 & 0 & random & 3/54 & 6/54 & & & & &  & \\
Alluxio & 3 & 0 & random & 4/54 & 4/54 & & & & &  & \\
Alluxio & 4 & 0 & random & 3/54 & 3/54 & & & & &  & \\
Alluxio & 5 & 0 & random & 0/54 & 4/54 & & & & &  & \\
Alluxio & 0 & 1 & random & 4/54 & 5/54 & & & & &  & \\
Alluxio & 1 & 1 & random & 3/54 & 10/54 & & & & &  & \\
Alluxio & 2 & 1 & random & 1/54 & 10/54 & & & & &  & \\
Alluxio & 3 & 1 & random & 1/54 & 4/54 & & & & &  & \\
Alluxio & 4 & 1 & random & 1/54 & 2/54 & & & & &  & \\
Alluxio & 0 & 2 & random & 0/54 & 6/54 & & & & &  & \\
Alluxio & 1 & 2 & random & 4/54 & 7/54 & & & & &  & \\
Alluxio & 2 & 2 & random & 5/54 & 4/54 & & & & &  & \\
Alluxio & 3 & 2 & random & 2/54 & 4/54 & & & & &  & \\
Alluxio & 0 & 3 & random & 2/54 & 2/54 & & & & &  & \\
Alluxio & 1 & 3 & random & 6/54 & 5/54 & & & & &  & \\
Alluxio & 2 & 3 & random & 7/54 & 3/54 & & & & &  & \\
Alluxio & 0 & 4 & random & 0/54 & 0/54 & & & & &  & \\
Alluxio & 1 & 4 & random & 5/54 & 2/54 & & 8/54 & 12/54 & &  & \\
Alluxio & 0 & 5 & random & 1/54 & 0/54 & & & & &  & \\
        \bottomrule
        \end{tabular}
        \caption{\llms still pinpoint the parameters with default values.}
\end{table*}


==> tables/project_description.tex <==
\vspace{5pt}
\begin{table}[ht]
    \footnotesize
    \setlength{\tabcolsep}{3pt}
    \centering
    \begin{tabular}{lllc}
      \toprule
      {\bf Software} & {\bf Module} & {\bf Release Time} & {\bf \#parameters} \\
      \midrule
      HCommon (2.8.5)   & {hadoop-common} & Sep, 2018    & 270    \\
      HBase (2.2.2)     & {hbase-server}  & Jul, 2019    & 204   \\
      Alluxio (2.1.0)   & {core}          & Nov, 2019    & 381    \\
      \bottomrule
    \end{tabular}
    \caption{Versions of the evaluated systems.}
    \label{tab:systemstatistics}
\end{table}


==> tables/relevant-shot.tex <==
\begin{table}[H]
    \vspace{3pt}
    \setlength{\tabcolsep}{3.7pt}
    \footnotesize
	\caption{Improvement in \paramlevel \fonescore when the misconfiguration in the evaluated file belongs to the same violation (sub-)category as the misconfiguration in the shot, compared to when they do not.}
    \centering
    \vspace{-5pt}
    \begin{tabular}{l|ccc|ccc}
        \toprule
        \multirow{2}{*}{\bf Models}  & \multicolumn{3}{c}{\bf Category}& \multicolumn{3}{c}{\bf Sub-Category}\\
        {}          & {\bf Diff.}   & {\bf Same} & {\bf \%Improv.}     & {\bf Diff.} & {\bf Same } & {\bf \%Improv.} \\
         \midrule
         {GPT-4}  & 0.57 & 0.65 & +12.9\% &0.60 & 0.57 & -5.3\%\\ 
        {GPT-3.5-turbo} & 0.41  & 0.53 & +28.2\%& 0.45 & 0.51 & +12.8\%\\ 
        {Code-Davinci-002}& 0.44  & 0.61 & +37.0\%& 0.48 &0.81 & +69.5\%\\
      \bottomrule
      \end{tabular}
      \vspace{5pt}
      \label{tab:releventShot}
\end{table}

==> tables/same-type.tex <==
\vspace{5pt}
\begin{table}[h]
  \footnotesize
  \setlength{\tabcolsep}{1.2pt}
  \centering
  \begin{tabular}{c|rrrr|rrr}
    \toprule
    \multirow{2}{*}{\bf } & \multicolumn{4}{c}{\bf \codedavinci} & \multicolumn{3}{c}{\bf \textdavinci} \\
    {} & {HCommon} & {HBase} & {Alluxio} & {} & {HCommon} & {HBase} & {Alluxio} \\
    \midrule
    {\% $CVC_{Original}$}  &  \oneHCommonCdCVC  & \oneHBaseCdCVC & \oneAlluxioCdCVC & {}                & \oneHCommonTdCVC & \oneHBaseTdCVC & \oneAlluxioTdCVC \\
    {\% $CVC_{SameType}$} &  \oneHCommonCdSameTypeCVC  & \oneHBaseCdSameTypeCVC & \oneAlluxioCdSameTypeCVC & {}         & \oneHCommonTdSameTypeCVC & \oneHBaseTdSameTypeCVC & \oneAlluxioTdSameTypeCVC \\
    \midrule
    {\% $CVC_{Improve}$} & \oneHCommonCdCVCImprovement & \oneHBaseCdCVCImprovement & \oneAlluxioCdCVCImprovement & {}        & \oneHCommonTdCVCImprovement & \oneHBaseTdCVCImprovement & \oneAlluxioTdCVCImprovement \\
    \midrule
    {\% $CVC_{AvgImprov}$}  & \multicolumn{3}{c}{\bf \oneavgCdCVCAvg} & {} &  \multicolumn{3}{c}{\bf \oneavgTdCVCAvg} \\
    \bottomrule
    \end{tabular}
    \caption{Improvement of LLMs when provided shot(s) contain \misconfigs that share the same root cause types as the \misconfig in the to-be-validated 
    \config change.}
    \label{tab:results:same-type}
\end{table}



% \newcommand{\oneHCommonCdSameTypeCVC}{64.00\xspace}
% \newcommand{\oneHCommonCdCVC}{53.41\xspace}
% \newcommand{\oneHCommonCdCVCImprovement}{10.59\xspace}
% \newcommand{\oneHCommonTdSameTypeCVC}{22.00\xspace}
% \newcommand{\oneHCommonTdCVC}{16.85\xspace}
% \newcommand{\oneHCommonTdCVCImprovement}{5.15\xspace}

% \newcommand{\oneHBaseCdSameTypeCVC}{60.27\xspace}
% \newcommand{\oneHBaseCdCVC}{49.61\xspace}
% \newcommand{\oneHBaseCdCVCImprovement}{10.66\xspace}
% \newcommand{\oneHBaseTdSameTypeCVC}{12.33\xspace}
% \newcommand{\oneHBaseTdCVC}{14.34\xspace}
% \newcommand{\oneHBaseTdCVCImprovement}{-2.01\xspace}

% \newcommand{\oneAlluxioCdSameTypeCVC}{47.54\xspace}
% \newcommand{\oneAlluxioCdCVC}{39.06\xspace}
% \newcommand{\oneAlluxioCdCVCImprovement}{8.48\xspace}
% \newcommand{\oneAlluxioTdSameTypeCVC}{34.43\xspace}
% \newcommand{\oneAlluxioTdCVC}{23.05\xspace}
% \newcommand{\oneAlluxioTdCVCImprovement}{11.38\xspace}

% \newcommand{\oneavgCdCVCAvg}{14.87\xspace}
% \newcommand{\oneavgTdCVCAvg}{7.26\xspace}

==> tables/shot.tex <==
\begin{table*}[h]
  \footnotesize
  \setlength{\tabcolsep}{3.75pt}
  \centering
  \begin{tabular}{p{0.4cm}l|rrrrr|rrrrr|rrrr}
    \toprule
    {} & \multirow{2}{*}{\bf } & \multicolumn{4}{c}{\bf \codedavinci} & & \multicolumn{4}{c}{\bf \codecushman} & & \multicolumn{4}{c}{\bf \textdavinci} \\
    {} & {} & {HCommon} & {HBase} & {Alluxio} & {$avg$} & & {HCommon} & {HBase} & {Alluxio} & {$avg$} & & {HCommon} & {HBase} & {Alluxio} & {$avg$} \\
    \midrule
    \rowcolor{LightGray}
    {} & \% CVC & \zeroHCommonCdCVC & \zeroHBaseCdCVC & \zeroAlluxioCdCVC & \zeroAvgCdCVC & & \zeroHCommonCcCVC & \zeroHBaseCcCVC & \zeroAlluxioCcCVC & \zeroAvgCcCVC & & \zeroHCommonTdCVC & \zeroHBaseTdCVC & \zeroAlluxioTdCVC & \zeroAvgTdCVC \\ 
    {} & \% Precision & \zeroHCommonCdPrecision & \zeroHBaseCdPrecision & \zeroAlluxioCdPrecision & \zeroAvgCdPrecision & & \zeroHCommonCcPrecision & \zeroHBaseCcPrecision & \zeroAlluxioCcPrecision & \zeroAvgCcPrecision & & \zeroHCommonTdPrecision & \zeroHBaseTdPrecision & \zeroAlluxioTdPrecision & \zeroAvgTdPrecision \\ 
    \multirow{3}{*}{\rotatebox{90}{\large \bf zero-shot}} & \% Recall & \zeroHCommonCdRecall & \zeroHBaseCdRecall & \zeroAlluxioCdRecall & \zeroAvgCdRecall & & \zeroHCommonCcRecall & \zeroHBaseCcRecall & \zeroAlluxioCcRecall & \zeroAvgCcRecall & & \zeroHCommonTdRecall & \zeroHBaseTdRecall & \zeroAlluxioTdRecall & \zeroAvgTdRecall \\ 
    {} & \% F1-score & \zeroHCommonCdF & \zeroHBaseCdF & \zeroAlluxioCdF & \zeroAvgCdF & & \zeroHCommonCcF & \zeroHBaseCcF & \zeroAlluxioCcF & \zeroAvgCcF & & \zeroHCommonTdF & \zeroHBaseTdF & \zeroAlluxioTdF & \zeroAvgTdF \\ 
    {} & \% Once & \zeroHCommonCdOnce & \zeroHBaseCdOnce & \zeroAlluxioCdOnce & \zeroAvgCdOnce & & \zeroHCommonCcOnce & \zeroHBaseCcOnce & \zeroAlluxioCcOnce & \zeroAvgCcOnce & & \zeroHCommonTdOnce & \zeroHBaseTdOnce & \zeroAlluxioTdOnce & \zeroAvgTdOnce \\ 
    {} & \% Majority & \zeroHCommonCdMajority & \zeroHBaseCdMajority & \zeroAlluxioCdMajority & \zeroAvgCdMajority & & \zeroHCommonCcMajority & \zeroHBaseCcMajority & \zeroAlluxioCcMajority & \zeroAvgCcMajority & & \zeroHCommonTdMajority & \zeroHBaseTdMajority & \zeroAlluxioTdMajority & \zeroAvgTdMajority \\ 
    {} & \% Everytime & \zeroHCommonCdEverytime & \zeroHBaseCdEverytime & \zeroAlluxioCdEverytime & \zeroAvgCdEverytime & & \zeroHCommonCcEverytime & \zeroHBaseCcEverytime & \zeroAlluxioCcEverytime & \zeroAvgCcEverytime & & \zeroHCommonTdEverytime & \zeroHBaseTdEverytime & \zeroAlluxioTdEverytime & \zeroAvgTdEverytime \\ 

    \midrule
    \rowcolor{LightGray}
    {} & \% CVC & \oneHCommonCdCVC & \oneHBaseCdCVC & \oneAlluxioCdCVC & \oneAvgCdCVC & & \oneHCommonCcCVC & \oneHBaseCcCVC & \oneAlluxioCcCVC & \oneAvgCcCVC & & \oneHCommonTdCVC & \oneHBaseTdCVC & \oneAlluxioTdCVC & \oneAvgTdCVC \\ 
    {} & \% Precision & \oneHCommonCdPrecision & \oneHBaseCdPrecision & \oneAlluxioCdPrecision & \oneAvgCdPrecision & & \oneHCommonCcPrecision & \oneHBaseCcPrecision & \oneAlluxioCcPrecision & \oneAvgCcPrecision & & \oneHCommonTdPrecision & \oneHBaseTdPrecision & \oneAlluxioTdPrecision & \oneAvgTdPrecision \\ 
    \multirow{3}{*}{\rotatebox{90}{\large \bf one-shot}} & \% Recall & \oneHCommonCdRecall & \oneHBaseCdRecall & \oneAlluxioCdRecall & \oneAvgCdRecall & & \oneHCommonCcRecall & \oneHBaseCcRecall & \oneAlluxioCcRecall & \oneAvgCcRecall & & \oneHCommonTdRecall & \oneHBaseTdRecall & \oneAlluxioTdRecall & \oneAvgTdRecall \\ 
    {} & \% F1-score & \oneHCommonCdF & \oneHBaseCdF & \oneAlluxioCdF & \oneAvgCdF & & \oneHCommonCcF & \oneHBaseCcF & \oneAlluxioCcF & \oneAvgCcF & & \oneHCommonTdF & \oneHBaseTdF & \oneAlluxioTdF & \oneAvgTdF \\ 
    {} & \% Once & \oneHCommonCdOnce & \oneHBaseCdOnce & \oneAlluxioCdOnce & \oneAvgCdOnce & & \oneHCommonCcOnce & \oneHBaseCcOnce & \oneAlluxioCcOnce & \oneAvgCcOnce & & \oneHCommonTdOnce & \oneHBaseTdOnce & \oneAlluxioTdOnce & \oneAvgTdOnce \\ 
    {} & \% Majority & \oneHCommonCdMajority & \oneHBaseCdMajority & \oneAlluxioCdMajority & \oneAvgCdMajority & & \oneHCommonCcMajority & \oneHBaseCcMajority & \oneAlluxioCcMajority & \oneAvgCcMajority & & \oneHCommonTdMajority & \oneHBaseTdMajority & \oneAlluxioTdMajority & \oneAvgTdMajority \\ 
    {} & \% Everytime & \oneHCommonCdEverytime & \oneHBaseCdEverytime & \oneAlluxioCdEverytime & \oneAvgCdEverytime & & \oneHCommonCcEverytime & \oneHBaseCcEverytime & \oneAlluxioCcEverytime & \oneAvgCcEverytime & & \oneHCommonTdEverytime & \oneHBaseTdEverytime & \oneAlluxioTdEverytime & \oneAvgTdEverytime \\ 

    \bottomrule
    \end{tabular}
    \caption{Effectiveness of Large Language Models in misconfiguration detection with zero-shot and one-shot.}
    \label{tab:results:shot}
\end{table*}


==> tables/strategy.tex <==
\begin{table*}[!htb]
    \setlength{\tabcolsep}{2pt}
    \tiny
    \centering
    \begin{tabular}{l|cccc|c|cccc|c}
        \toprule
        \multirow{2}{*}{\bf Models} & \multicolumn{5}{c}{\bf F1-score (File Level)} & \multicolumn{5}{c}{\bf F1-score (Param Level)} \\
         & Rand. & Diff-Cat. & Sim. & Diff-Cat.+Sim. & \textbf{Avg} & Rand. & Diff-Cat. & Sim. & Diff-Cat.+Sim. & \textbf{Avg} \\
         \midrule
        {GPT-4} & - & - & - & - & - & - & - & - & - & - \\
        {GPT-3.5-turbo} & - & - & - & - & - & - & - & - & - & - \\
        {Code-Davinci-002} & - & - & - & - & - & - & - & - & - & - \\
      \bottomrule
      \end{tabular}
      \caption{Effectiveness of \llms for different strategies.}
      \label{tab:strategies}
\end{table*}


==> tables/temperature.tex <==
\begin{table}[ht]
    \footnotesize
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}{c|rrrrrrr}
      \toprule 
      {Temp} & {\% CVC} & {\% Precision} & {\% Recall} & {\% F1-Score} & {\% Once} & {\% Major} & {\% Every}\\
      \midrule
      0.1 & \cellcolor{LightGray}\zeroHCommonCdZponeCVC & \cellcolor{VeryLightGray}\zeroHCommonCdZponePrecision & \zeroHCommonCdZponeRecall & \cellcolor{LightGray}\zeroHCommonCdZponeF & \cellcolor{VeryLightGray}\zeroHCommonCdZponeOnce & \cellcolor{LightGray}\zeroHCommonCdZponeMajority & \cellcolor{LightGray}\zeroHCommonCdZponeEverytime \\ 
      0.2 & \zeroHCommonCdZptwoCVC & \zeroHCommonCdZptwoPrecision & \zeroHCommonCdZptwoRecall & \zeroHCommonCdZptwoF & \zeroHCommonCdZptwoOnce & \zeroHCommonCdZptwoMajority & \zeroHCommonCdZptwoEverytime \\ 
      0.3 & \zeroHCommonCdZpthreeCVC & \zeroHCommonCdZpthreePrecision & \zeroHCommonCdZpthreeRecall & \zeroHCommonCdZpthreeF & \zeroHCommonCdZpthreeOnce & \zeroHCommonCdZpthreeMajority & \zeroHCommonCdZpthreeEverytime \\ 
      0.4 & \cellcolor{LightGray}\zeroHCommonCdZpfourCVC & \cellcolor{LightGray}\zeroHCommonCdZpfourPrecision & \zeroHCommonCdZpfourRecall & \cellcolor{LightGray}\zeroHCommonCdZpfourF & \cellcolor{LightGray}\zeroHCommonCdZpfourOnce & \cellcolor{VeryLightGray}\zeroHCommonCdZpfourMajority & \cellcolor{VeryLightGray}\zeroHCommonCdZpfourEverytime \\ 
      0.5 & \zeroHCommonCdZpfiveCVC & \zeroHCommonCdZpfivePrecision & \zeroHCommonCdZpfiveRecall & \zeroHCommonCdZpfiveF & \zeroHCommonCdZpfiveOnce & \zeroHCommonCdZpfiveMajority & \zeroHCommonCdZpfiveEverytime \\ 
      0.6 & \zeroHCommonCdZpsixCVC & \zeroHCommonCdZpsixPrecision & \zeroHCommonCdZpsixRecall & \zeroHCommonCdZpsixF & \zeroHCommonCdZpsixOnce & \zeroHCommonCdZpsixMajority & \zeroHCommonCdZpsixEverytime \\ 
      0.7 & \zeroHCommonCdZpsevenCVC & \zeroHCommonCdZpsevenPrecision & \zeroHCommonCdZpsevenRecall & \zeroHCommonCdZpsevenF & \zeroHCommonCdZpsevenOnce & \zeroHCommonCdZpsevenMajority & \zeroHCommonCdZpsevenEverytime \\ 
      0.8 & \zeroHCommonCdZpeightCVC & \zeroHCommonCdZpeightPrecision & \zeroHCommonCdZpeightRecall & \zeroHCommonCdZpeightF & \zeroHCommonCdZpeightOnce & \zeroHCommonCdZpeightMajority & \zeroHCommonCdZpeightEverytime \\ 
      0.9 & \zeroHCommonCdZpnineCVC & \zeroHCommonCdZpninePrecision & \zeroHCommonCdZpnineRecall & \zeroHCommonCdZpnineF & \zeroHCommonCdZpnineOnce & \zeroHCommonCdZpnineMajority & \zeroHCommonCdZpnineEverytime \\ 
      1.0 & \zeroHCommonCdZptenCVC & \zeroHCommonCdZptenPrecision & \zeroHCommonCdZptenRecall & \zeroHCommonCdZptenF & \zeroHCommonCdZptenOnce & \zeroHCommonCdZptenMajority & \zeroHCommonCdZptenEverytime \\
      \bottomrule
      \end{tabular}
      \caption{Effectiveness of \itcodedavinci in misconfiguration detection with different temperature of zero-shot setting on \hcommon dataset.}
      \label{tab:results:diff-temp}
\end{table}

==> tables/zeroshot.tex <==
\begin{table*}[h]
  \footnotesize
  \setlength{\tabcolsep}{4.2pt}
  \centering
  \begin{tabular}{l|rrrrr|rrrrr|rrrr}
    \toprule
    \multirow{2}{*}{\bf } & \multicolumn{4}{c}{\bf \codedavinci} & & \multicolumn{4}{c}{\bf \codecushman} & & \multicolumn{4}{c}{\bf \textdavinci} \\
    {} & {HCommon} & {HBase} & {Alluxio} & {$avg$} & & {HCommon} & {HBase} & {Alluxio} & {$avg$} & & {HCommon} & {HBase} & {Alluxio} & {$avg$} \\
    \midrule

    
    \# CA & \zeroHCommonCdCA & \zeroHBaseCdCA & \zeroAlluxioCdCA & \zeroAvgCdCA & & \zeroHCommonCcCA & \zeroHBaseCcCA & \zeroAlluxioCcCA & \zeroAvgCcCA & & \zeroHCommonTdCA & \zeroHBaseTdCA & \zeroAlluxioTdCA & \zeroAvgTdCA \\ 
    \# WA & \zeroHCommonCdWA & \zeroHBaseCdWA & \zeroAlluxioCdWA & \zeroAvgCdWA & & \zeroHCommonCcWA & \zeroHBaseCcWA & \zeroAlluxioCcWA & \zeroAvgCcWA & & \zeroHCommonTdWA & \zeroHBaseTdWA & \zeroAlluxioTdWA & \zeroAvgTdWA \\ 
    \# EA & \zeroHCommonCdEA & \zeroHBaseCdEA & \zeroAlluxioCdEA & \zeroAvgCdEA & & \zeroHCommonCcEA & \zeroHBaseCcEA & \zeroAlluxioCcEA & \zeroAvgCcEA & & \zeroHCommonTdEA & \zeroHBaseTdEA & \zeroAlluxioTdEA & \zeroAvgTdEA \\ 
    \% Precision & \zeroHCommonCdPrecision & \zeroHBaseCdPrecision & \zeroAlluxioCdPrecision & \zeroAvgCdPrecision & & \zeroHCommonCcPrecision & \zeroHBaseCcPrecision & \zeroAlluxioCcPrecision & \zeroAvgCcPrecision & & \zeroHCommonTdPrecision & \zeroHBaseTdPrecision & \zeroAlluxioTdPrecision & \zeroAvgTdPrecision \\ 
    \% CVC & \zeroHCommonCdCVC & \zeroHBaseCdCVC & \zeroAlluxioCdCVC & \zeroAvgCdCVC & & \zeroHCommonCcCVC & \zeroHBaseCcCVC & \zeroAlluxioCcCVC & \zeroAvgCcCVC & & \zeroHCommonTdCVC & \zeroHBaseTdCVC & \zeroAlluxioTdCVC & \zeroAvgTdCVC \\ 
    \% Once & \zeroHCommonCdOnce & \zeroHBaseCdOnce & \zeroAlluxioCdOnce & \zeroAvgCdOnce & & \zeroHCommonCcOnce & \zeroHBaseCcOnce & \zeroAlluxioCcOnce & \zeroAvgCcOnce & & \zeroHCommonTdOnce & \zeroHBaseTdOnce & \zeroAlluxioTdOnce & \zeroAvgTdOnce \\ 
    \% Majority & \zeroHCommonCdMajority & \zeroHBaseCdMajority & \zeroAlluxioCdMajority & \zeroAvgCdMajority & & \zeroHCommonCcMajority & \zeroHBaseCcMajority & \zeroAlluxioCcMajority & \zeroAvgCcMajority & & \zeroHCommonTdMajority & \zeroHBaseTdMajority & \zeroAlluxioTdMajority & \zeroAvgTdMajority \\ 
    \% Everytime & \zeroHCommonCdEverytime & \zeroHBaseCdEverytime & \zeroAlluxioCdEverytime & \zeroAvgCdEverytime & & \zeroHCommonCcEverytime & \zeroHBaseCcEverytime & \zeroAlluxioCcEverytime & \zeroAvgCcEverytime & & \zeroHCommonTdEverytime & \zeroHBaseTdEverytime & \zeroAlluxioTdEverytime & \zeroAvgTdEverytime \\

    \bottomrule
    \end{tabular}
    \caption{Effectiveness of Large Language Models in misconfiguration detection without shots.}
    \label{tab:results:zero-shot}
\end{table*}

